Deep learning enables reference-free isotropic super-resolution for volumetric fluorescence microscopy

Volumetric imaging by fluorescence microscopy is often limited by anisotropic spatial resolution from inferior axial resolution compared to the lateral resolution. To address this problem, here we present a deep-learning-enabled unsupervised super-resolution technique that enhances anisotropic images in volumetric fluorescence microscopy. In contrast to the existing deep learning approaches that require matched high-resolution target volume images, our method greatly reduces the effort to put into practice as the training of a network requires as little as a single 3D image stack, without a priori knowledge of the image formation process, registration of training data, or separate acquisition of target data. This is achieved based on the optimal transport driven cycle-consistent generative adversarial network that learns from an unpaired matching between high-resolution 2D images in lateral image plane and low-resolution 2D images in the other planes. Using fluorescence confocal microscopy and light-sheet microscopy, we demonstrate that the trained network not only enhances axial resolution, but also restores suppressed visual details between the imaging planes and removes imaging artifacts.

==> 2021 Nature Comm A2L_arxiv-version/macros.tex <==
% macros.tex
% useful macros (shortcuts) to save typing

\newcommand{\add}[1] {\textcolor{blue}{#1}} % for revision
\newcommand{\addmore}[1] {\textcolor{red}{#1}} % for revision

\newtheorem{theorem}{\bf{Theorem}}
\newtheorem{lemma}{\bf{Lemma}}
\newtheorem{proposition}{\bf{Proposition}}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{\bf{Definition}}
\newtheorem{remark}{\bf{Remark}}
\newtheorem{example}{\bf{Example}}
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\renewenvironment{proof}{\emph{Proof.}}{\hfill\QED}

% now define useful macros

\long\def\comment#1{} % comment out text
\newcommand{\term}[1] {\emph{#1}}
\newcommand{\reg} {\xmath{\beta}}

\newcommand{\fref}[1] {Fig.~\ref{#1}\xspace}
\newcommand{\tref}[1]{Table~\ref{#1}}

\DeclareMathOperator*{\argminop}{arg\,min} % thin space, limits underneath
\def\argmin#1{\argminop_{#1}}
%\newcommand{\argmin}{\operatorname{argmin}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\st}{\operatorname{s.t.}}
\newcommand{\range}{\operatorname{Range}}
\newcommand{\rank}{\operatorname{rank}}
\renewcommand{\dim}{\operatorname{dim}}
\newcommand{\pri}{\text{pri}}
\newcommand{\dual}{\text{dual}}

\newcommand{\bmat}[1] {\begin{bmatrix} #1 \end{bmatrix}} % best arrays ever

\newcommand{\xmath}[1] {\ensuremath{#1}\xspace}
\newcommand{\blmath}[1] {\xmath{\bm{#1}}}
\newcommand{\A}{\blmath{A}}
\newcommand{\B}{\blmath{B}}
\newcommand{\C}{\blmath{C}}
\newcommand{\D}{\blmath{D}}
\newcommand{\E}{\blmath{E}}
\newcommand{\F}{\blmath{F}}
\newcommand{\I}{\blmath{I}}
\newcommand{\R}{\blmath{R}}
\newcommand{\T}{\blmath{T}}
\newcommand{\U}{\blmath{U}}
\newcommand{\V}{\blmath{V}}
\newcommand{\W}{\blmath{W}}
\newcommand{\X}{\blmath{X}}
\newcommand{\Y}{\blmath{Y}}
\newcommand{\Z}{\blmath{Z}}
%%
%Sai's Macros
\renewcommand{\P}{\blmath{P}} % todo: some problem here...
\renewcommand{\H}{\blmath{H}}
\newcommand{\G}{\blmath{G}}
%\newcommand{\z}{\blmath{z}}
%%

\newcommand{\x}{\blmath{x}}
\newcommand{\xh}{\xmath{\hat{\x}}}
\newcommand{\y}{\blmath{y}}
\newcommand{\z}{\blmath{z}}
\newcommand{\zh}{\xmath{\hat{\z}}}
\newcommand{\1}{\blmath{1}} 
\newcommand{\0}{\blmath{0}} 
\renewcommand{\Re}{\mathbb{R}}
\newcommand{\ie}{\text{i.e.}}
\newcommand{\eg}{\text{e.g.}}

\newcommand{\bLam}{\blmath{\Lambda}}

\newcommand{\norm}[1] {\xmath{\left\| #1 \right\|}}
\newcommand{\normi}[1] {\xmath{\left\| #1 \right\|_1}}
\newcommand{\normii}[1] {\xmath{\left\| #1 \right\|_2}}


%%% Jong's macros

\newcommand{\Cm}{{\mathcal C}}
\newcommand{\Ab}{{\blmath A}}
\newcommand{\Bb}{{\blmath B}}
\newcommand{\Cb}{{\blmath{C}}}
\newcommand{\Db}{{\blmath D}}
\newcommand{\Eb}{{\blmath E}}
\newcommand{\Fb}{{\blmath F}}
\newcommand{\Gb}{{\blmath G}}
\newcommand{\Hb}{{\blmath H}}
\newcommand{\Ib}{{\blmath I}}
\newcommand{\Jb}{{\blmath J}}
\newcommand{\Kb}{{\blmath K}}
\newcommand{\Lb}{{\blmath L}}
\newcommand{\Mb}{{\blmath M}}
\newcommand{\Nb}{{\blmath N}}
\newcommand{\Ob}{{\blmath O}}
\newcommand{\Pb}{{\blmath P}}
\newcommand{\Qb}{{\blmath Q}}
\newcommand{\Rb}{{\blmath R}}
\newcommand{\Sb}{{\blmath S}}
\newcommand{\Tb}{{\blmath T}}
\newcommand{\Ub}{{\blmath U}}
\newcommand{\Vb}{{\blmath V}}
\newcommand{\Wb}{{\blmath W}}
\newcommand{\Xb}{{\blmath X}}
\newcommand{\Yb}{{\blmath Y}}
\newcommand{\Zb}{{\blmath Z}}

\newcommand{\ab}{{\blmath a}}
\newcommand{\bb}{{\blmath b}}
\newcommand{\cb}{{\blmath c}}
\newcommand{\db}{{\blmath d}}
\newcommand{\eb}{{\blmath e}}
\newcommand{\fb}{{\blmath f}}
\newcommand{\gb}{{\blmath g}}
\newcommand{\hb}{{\blmath h}}
\newcommand{\ib}{{\blmath i}}
\newcommand{\jb}{{\blmath j}}
\newcommand{\kb}{{\blmath k}}
\newcommand{\lb}{{\blmath l}}
\newcommand{\mb}{{\blmath m}}
\newcommand{\nb}{{\blmath n}}
\newcommand{\ob}{{\blmath o}}
\newcommand{\pb}{{\blmath p}}
\newcommand{\qb}{{\blmath q}}
\newcommand{\rb}{{\blmath r}}
\renewcommand{\sb}{{\blmath s}}
\newcommand{\tb}{{\blmath t}}
\newcommand{\ub}{{\blmath u}}
\newcommand{\vb}{{\blmath v}}
\newcommand{\wb}{{\blmath w}}
\newcommand{\xb}{{\blmath x}}
\newcommand{\yb}{{\blmath y}}
\newcommand{\zb}{{\blmath z}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\mbf}{\blmath}
\newcommand{\bs}{\boldsymbol}
% sentence
\newcommand{\Hs}{\mathscr{H}}
\newcommand{\Xs}{\mathscr{X}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Zc}{\mathcal{Z}}
\newcommand{\Vc}{\mathcal{V}}
\newcommand{\Wc}{\mathcal{W}}

\newcommand{\Phib}{{\boldsymbol {\Phi}}}
\newcommand{\Psib}{{\boldsymbol {\Psi}}}
\newcommand{\Thetab}{{\boldsymbol {\Theta}}}
%\newcommand{\Lambda_b}{{\boldsymbol {\Lambda}}}
\newcommand{\Xib}{{\boldsymbol {\Xi}}}
\newcommand{\Sigmab}{{\boldsymbol {\Sigma}}}
\newcommand{\Rd}{{\mathbb R}}
\newcommand{\Cd}{{\mathbb C}}
\newcommand{\deltab}{{\boldsymbol{\delta}}}
\newcommand{\mub}{{\boldsymbol{\mu}}}
\newcommand{\nub}{{\boldsymbol{\nu}}}
\newcommand{\phib}{{\boldsymbol{\phi}}}
\newcommand{\psib}{{\boldsymbol{\psi}}}
\newcommand{\rhob}{{\boldsymbol {\rho}}}
\newcommand{\alphab}{{\boldsymbol {\alpha}}}
%\newcommand{\0}{{\boldsymbol{0}}}
%\newcommand{\Xbc}{{\boldsymbol{\cal X}}}
\newcommand{\Lbc}{{\boldsymbol{\mathcal L}}}
\newcommand{\Ybc}{{\boldsymbol{\mathcal Y}}}
\newcommand{\Sbc}{{\boldsymbol{\mathcal S}}}
\newcommand{\Qbc}{{\boldsymbol{\mathcal Q}}}
\newcommand{\Pbc}{{\boldsymbol{\mathcal P}}}
\newcommand{\Rbc}{{\boldsymbol{\mathcal R}}}
\newcommand{\Zbc}{{\boldsymbol{\mathcal Z}}}
\newcommand{\Abc}{{\boldsymbol{\mathcal A}}}
\newcommand{\Ebc}{{\boldsymbol{\mathcal E}}}
\newcommand{\Cbc}{{\boldsymbol{\mathcal C}}}
\newcommand{\Dbc}{{\boldsymbol{\mathcal D}}}
\newcommand{\thetab}{{\boldsymbol {\theta}}}
\newcommand{\chib}{{\boldsymbol {\chi}}}
\newcommand{\Hbc}{{\boldsymbol{\mathcal H}}}
\newcommand{\Xbc}{{\boldsymbol{\mathcal X}}}
\newcommand{\Kbc}{{\boldsymbol{\mathcal K}}}
\newcommand{\Mbc}{{\boldsymbol{\mathcal M}}}
\newcommand{\Kc}{{{\mathcal K}}}
\newcommand{\Pc}{{{\mathcal P}}}
\newcommand{\Ec}{{{\mathcal E}}}
\newcommand{\Dc}{{{\mathcal D}}}

\newcommand{\Ed}{{{\mathbb E}}}
\newcommand{\Zd}{\mathbb{Z}}
%\newcommand{\rank}{\mathrm{rank}}
\newcommand{\hank}{\boldsymbol{\mathbb{H}}}
\newcommand{\cir}{\mathscr{C}}
\newcommand{\conv}{\boldsymbol{\mathbb{C}}}
\newcommand{\Tconv}{\mathcal{T}}
\newcommand{\zerob}{\mathbf{0}}
\newcommand{\hbk}{\boldsymbol{\mathfrak{h}}}
\newcommand{\Null}{\textsc{Nul}}
\newcommand{\Ran}{\textsc{Ran}}
%\newcommand{\rank}{\textsc{rank}}
\newcommand{\id}{\mathrm{id}}

\newcommand{\Md}{\mathbb{M}}
\newcommand{\Kd}{\mathbb{K}}
\newcommand{\Jd}{\mathbb{J}}
\newcommand{\Td}{\mathbb{T}}
%%%
\newcommand{\imsize}{6.5}
\newcommand{\imsizer}{6.2}
\newcommand{\imsizeh}{3.2}
\newcommand{\imsizes}{4}



%%%%%%%%%%
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\Fc}{{\mathcal F}}

\newcommand{\vect}{\textsc{Vec}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\Lambdab}{\boldsymbol{\Lambda}}

==> 2021 Nature Comm A2L_arxiv-version/packages.tex <==
% packages.tex
% load a lot of possibly useful packages
% all of these are documented on web sites online

\usepackage{outline}
\usepackage{pmgraph}
\usepackage[normalem]{ulem}
\usepackage[utf8]{inputenc}
%\usepackage{gensymb}
\usepackage{amssymb}
\usepackage{hyperref}
\usepackage{amsmath}
\usepackage{graphicx}
%\usepackage[text={6.5in,9in},centering]{geometry}
%%%
\usepackage{times}
\usepackage{xcolor}
\usepackage{xspace}
\usepackage[colorinlistoftodos]{todonotes} % for \todo
\usepackage{cite}
\usepackage{bm} % bold
%\setlength{\parskip}{1em}
%\setlength{\parindent}{0em}
%%%
%\usepackage[font=footnotesize,labelfont=bf]{caption}
%\usepackage[font=footnotesize,labelfont=bf]{subcaption}
%\usepackage{subcaption}
\usepackage{url}

\usepackage{epstopdf}
%\epstopdfDeclareGraphicsRule{.tiff}{png}{.png}{convert #1 \OutputFile}
\AppendGraphicsExtensions{.tiff}
\graphicspath{{fig/}} % Directory in which figures are stored

\usepackage{epsfig}
\usepackage{tikz}
\usetikzlibrary{spy}
\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{mathrsfs}

%% Sungjoon

\usepackage{amsmath,graphicx,caption,mathtools,amssymb,amsthm}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{subcaption}
\usepackage{accents}
%\usepackage{txfonts}
% \usepackage{eucal}

%\addbibresource{refs_jcy.bib}
